Worm Algorithm for CP(N-1) Model

The CP(N-1) model in 2D is an interesting toy model for 4D QCD as it possesses confinement, asymptotic freedom and a non-trivial vacuum structure. Due to the lower dimensionality and the absence of fermions, the computational cost for simulating 2D CP(N-1) on the lattice is much lower than that for simulating 4D QCD. However, to our knowledge, no efficient algorithm for simulating the lattice CP(N-1) model has been tested so far, which also works at finite density. To this end we propose a new type of worm algorithm which is appropriate to simulate the lattice CP(N-1) model in a dual, flux-variables based representation, in which the introduction of a chemical potential does not give rise to any complications. In addition to the usual worm moves where a defect is just moved from one lattice site to the next, our algorithm additionally allows for worm-type moves in the internal variable space of single links, which accelerates the Monte Carlo evolution. We use our algorithm to compare the two popular CP(N-1) lattice actions and exhibit marked differences in their approach to the continuum limit.

==> tikzimg/mcprobabs.tex <==
\DeclareRobustCommand\tkboxa{
\begin{tikzpicture}[scale=0.3,nodes={inner sep=0}]
  \pgfpointtransformed{\pgfpointxy{1}{1}};
  \pgfgetlastxy{\vx}{\vy}
  \begin{scope}[node distance=\vx and \vy]
    \def\xa{0};
    \def\ya{0};
    \foreach \i in {1,...,5} {
        \draw [thin,dotted,gray] (\xa+\i,\ya+1) -- (\xa+\i,\ya+5) node[solid,black,above] at (\xa+\i,\ya+5.3) {};
    }
    \foreach \i in {1,...,5} {
        \draw [thin,dotted,gray] (\xa+1,\ya+\i) -- (\xa+5,\ya+\i) node[solid,black,left] at (\xa+0.7,\ya+6-\i) {};
    }
    \foreach \i in {1,...,5} {
      \draw [thin,black!100] (\xa+5,\ya+6-\i) -- (\xa+\i,\ya+6-\i) -- (\xa+\i,\ya+6-1);
    }
    \draw [thin,dashed,black] (\xa+1,\ya+5) -- (\xa+5,\ya+1);

    
    \def\pxa{4};
    \def\pya{3};
    \node[left,scale=0.65] at (\xa+0.75,\ya+6-\pya) {$a_{0}$};
    \draw [thin,black] (\xa+0.85,\ya+6-\pya) -- (\xa+1,\ya+6-\pya);
    \node[left,scale=0.65] at (\xa+0.75,\ya+6-\pxa) {$b_{0}$};
    \draw [thin,black] (\xa+0.85,\ya+6-\pxa) -- (\xa+1,\ya+6-\pxa);
    \draw [thin,dotted,red] (\xa+\pxa+0.1,\ya+6-\pya-0.1) -- (\xa+\pya+0.1,\ya+6-\pxa-0.1);
    \draw [thin,dotted,red] (\xa+\pxa-0.1,\ya+6-\pya+0.1) -- (\xa+\pya-0.1,\ya+6-\pxa+0.1);
	\node[draw,thick,cross,inner sep=1.5,color=red] at (\xa+\pxa+0.1,\ya+6-\pya-0.1) {};
	\node[draw,thick,cross,rotate=45,inner sep=1.5,color=red] at (\xa+\pya+0.1,\ya+6-\pxa-0.1) {};
	\node[draw,thick,cross,rotate=45,inner sep=1.5,color=red] at (\xa+\pxa-0.1,\ya+6-\pya+0.1) {};
	\node[draw,thick,cross,inner sep=1.5,color=red] at (\xa+\pya-0.1,\ya+6-\pxa+0.1) {};
  \end{scope}
\end{tikzpicture}
}

\begin{tikzpicture}[scale=0.8,nodes={inner sep=0}]
  \pgfpointtransformed{\pgfpointxy{1}{1}};
  \pgfgetlastxy{\vx}{\vy}
  \begin{scope}[node distance=\vx and \vy]
    \node[scale=0.8] at (-4,3.2) {$Z$};
    \draw[->] (-3.3,4.2) to[bend left] node[pos=0.5,above=0.1,scale=0.75]{$\sfrac{1}{\of{V\,N\,\of{N-1}}}$} (-0.7,4.2);
    \draw[<-] (-3.3,3.8) to[bend right] node[pos=0.5,below=0.1,scale=0.75]{$\sfrac{1}{2}$} (-0.7,3.8);
  \end{scope}
  
  \begin{scope}[node distance=\vx and \vy]
    \node[align=center,label=below:\scalebox{0.75}{$x_{0}$}] at (0,4) {\tkboxa};
    \node[scale=0.8] at (0,3.2) {$Z_{2}^{a_{0}\,b_{0}}\of{x_{0},x_{0}}$};
  \end{scope}
  
  \begin{scope}[node distance=\vx and \vy]
    \node[draw,circle,inner sep=1.2,thick,color=red,fill=red,outer sep=1.6,label=below:{\scalebox{0.75}{$x_{0}$}}] at (3.95,4) {};
    \node[draw,circle,inner sep=1.2,thick,color=red,fill=white,outer sep=1.6,label=below:{\scalebox{0.75}{$x$}}] at (5.05,4) {};
    \draw[-,ultra thick,color=red] (4.075,4) -- (4.925,4);
    \node[scale=0.8] at (4.6,3.2) {$Z_{2}^{2\,1}\of{x_{0},x}$};

    \draw[->] (0.7,4.2) to[bend left] node[pos=0.5,above=0.1,scale=0.75]{$\sfrac{1}{\of{2\,u}}$} (3.3,4.2);
    \draw[<-] (0.7,3.8) to[bend right] node[pos=0.5,below=0.1,scale=0.75]{$\sfrac{1}{u}$} (3.3,3.8);
  \end{scope}
  
  \begin{scope}[node distance=\vx and \vy]
    \node[draw,circle,inner sep=1.2,thick,color=red,fill=red,outer sep=1.6,label=below:{\scalebox{0.75}{$x_{0}$}}] at (-0.1,8) {};
    \node[draw,circle,inner sep=1.2,thick,color=blue,fill=white,outer sep=1.6] at (0.1,8) {};
    \node[draw,circle,inner sep=1.2,thick,color=darkgreen,fill=white,outer sep=1.6,label=below:{\scalebox{0.75}{$y$}}] at (1.1,9) {};
    \node[draw,circle,inner sep=1.2,thick,color=darkyellow,fill=darkyellow,outer sep=1.6] at (0.9,9) {};
    \node[scale=0.8] at (0,9.5) {$Z_{2}^{2\,3}\of{x_{0},y}$};

    \draw[->] (-0.2,4.7) to[bend left] node[pos=0.5,left=0.1,scale=0.75]{$\sfrac{1}{\of{2\,u\,\of{V-1}}}$} (-0.2,7.3);
    \draw[<-] (0.2,4.7) to[bend right] node[pos=0.5,right=0.1,scale=0.75]{$\sfrac{1}{\of{u\,\of{V-1}}}$} (0.2,7.3);
  \end{scope}
\end{tikzpicture}
